Compressing Sentence Representation with maximum Coding Rate Reduction

In most natural language inference problems, sentence representation is needed for semantic retrieval tasks. In recent years, pre-trained large language models have been quite effective for computing such representations. These models produce high-dimensional sentence embeddings. An evident performance gap between large and small models exists in practice. Hence, due to space and time hardware limitations, there is a need to attain comparable results when using the smaller model, which is usually a distilled version of the large language model. In this paper, we assess the model distillation of the sentence representation model Sentence-BERT by augmenting the pre-trained distilled model with a projection layer additionally learned on the Maximum Coding Rate Reduction (MCR2)objective, a novel approach developed for general-purpose manifold clustering. We demonstrate that the new language model with reduced complexity and sentence embedding size can achieve comparable results on semantic retrieval benchmarks.

==> MCR Sentence Representation Compression (ArXiv)/gfx/results.tex <==

\begin{table*}[!h]
\scriptsize
    \caption{\small For Semantic Retrieval (SR) tasks the \texttt{all-mpnet-base-v2} SBERT model with MCR$^2$ projection to dimension 200 achieves best accuracy without no additional time for clustering like in the same setup with $k$-means (denoted with $^{*}$). Clustering backbone sentence embeddings from SBERT with $k$-means (denoted with $^{**}$) took almost an hour.}
    \label{tab:SR_results}
    \centering
\begin{tabular}{lr|lll}
\toprule
                                        &           &          \multicolumn{3}{c}{\sc Time} \\
                                   model &  accuracy & encoding & clustering &    total \\
\midrule
 all-mpnet-base-v2 + MCR50  &     0.562 & 00:04:15 &      -      & 00:04:15 \\
all-mpnet-base-v2 + MCR100  &     0.545 & 00:04:15 &      -     & 00:04:15 \\
\textbf{all-mpnet-base-v2 + MCR200}  &     0.645 & 00:04:16 &      -     & 00:04:16 \\
all-mpnet-base-v2 + MCR300  &     0.632 & 00:04:17 &      -     & 00:04:17 \\
    \midrule
    
all-mpnet-base-v2 + MCR50 + kmeans &     0.671 & 00:04:15 &   00:07:08 & 00:11:23 \\
all-mpnet-base-v2 + MCR100 + kmeans &     0.650 & 00:04:15 &   00:07:22 & 00:11:37 \\
all-mpnet-base-v2 + MCR200 + kmeans$^{*}$ &     0.635 & 00:04:16 &   00:09:08 & 00:13:24 \\
all-mpnet-base-v2 + MCR300 + kmeans &     0.631 & 00:04:17 &   00:11:09 & 00:15:26 \\
all-mpnet-base-v2 + kmeans (768)$^{**}$ &     0.648 & 00:04:17 &   00:59:57 & 01:04:12 \\
all-mpnet-base-v2 + MCR768 + kmeans 	&  	0.630 	&	00:04:17 &	00:18:15 & 	00:22:32	\\
\bottomrule
\end{tabular}
\end{table*}



\begin{table*}[!h]
\scriptsize
    \caption{\small For Semantic Textual Similarity (STS) tasks backbone model achieves the best results (bolded) for Spearman rank correlation coefficient on multiple benchmarks, although we observe comparable results of our method compared to the backbone and distilled model \texttt{all-MiniLM-L6-v2}.}
    \label{tab:STS_results}
    \centering
\begin{tabular}{lrrrrrr}
\toprule
                      model &  STSb &  STS12 &  STS13 &  STS14 &  STS15 &  STS16 \\
\midrule
 all-mpnet-base-v2 + MCR50 & 0.749 &  0.666 &  0.739 &  0.713 &  0.754 &  0.768 \\
all-mpnet-base-v2 + MCR100 & 0.788 &  0.696 &  0.782 &  0.753 &  0.791 &  0.793 \\
all-mpnet-base-v2 + MCR200 & 0.818 &  0.712 &  0.812 &  0.779 &  0.819 &  0.816 \\
all-mpnet-base-v2 + MCR300 & 0.821 &  0.718 &  0.817 &  0.783 &  0.827 &  0.823 \\
\textbf{all-mpnet-base-v2 (768)} & 0.836 &  0.722 &  0.821 &  0.790 &  0.838 &  0.831 \\
\midrule
  all-MiniLM-L6-v2 + MCR50 & 0.752 &  0.654 &  0.690 &  0.682 &  0.741 &  0.737 \\
 all-MiniLM-L6-v2 + MCR100 & 0.778 &  0.685 &  0.742 &  0.721 &  0.780 &  0.777 \\
 all-MiniLM-L6-v2 + MCR200 & 0.810 &  0.705 &  0.773 &  0.751 &  0.813 &  0.792 \\
 all-MiniLM-L6-v2 + MCR300 & 0.813 &  0.710 &  0.780 &  0.759 &  0.826 &  0.800 \\
\textbf{all-MiniLM-L6-v2 (384)} & 0.824 &  0.711 &  0.790 &  0.772 &  0.838 &  0.812 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!h]
\scriptsize
    \caption{\small For Sentence Classification (SC) tasks backbone model achieves the best results (bolded) for accuracy on multiple benchmarks, although we observe comparable results of our method compared to the backbone and distilled model.}
    \label{tab:SC_results}
    \centering
\begin{tabular}{lrrrrrrr}
\toprule
                      model &  SST2 &  SST5 &    MR &    CR &  SUBJ &  MPQA &  TREC \\
\midrule
 all-mpnet-base-v2 + MCR50 & 75.45 & 36.43 & 69.67 & 63.76 & 79.16 & 68.84 &  51.6 \\
all-mpnet-base-v2 + MCR100 & 82.54 & 39.19 & 75.85 & 63.76 & 81.86 & 68.77 &  60.0 \\
all-mpnet-base-v2 + MCR200 & 86.55 & 42.76 & 80.62 & 72.77 & 88.28 & 82.27 &  71.0 \\
all-mpnet-base-v2 + MCR300 & 87.59 & 44.66 & 82.33 & 79.71 & 90.73 & 85.76 &  79.8 \\
         \textbf{all-mpnet-base-v2 (768)} & 88.74 & 49.00 & 85.05 & 86.84 & 93.97 & 89.32 &  94.0 \\
\midrule
  all-MiniLM-L6-v2 + MCR50 & 65.95 & 31.76 & 61.61 & 63.76 & 79.19 & 68.77 &  41.0 \\
 all-MiniLM-L6-v2 + MCR100 & 72.27 & 33.94 & 66.38 & 63.82 & 83.97 & 76.58 &  64.0 \\
 all-MiniLM-L6-v2 + MCR200 & 77.54 & 37.10 & 70.06 & 69.17 & 86.87 & 81.83 &  69.2 \\
 all-MiniLM-L6-v2 + MCR300 & 79.35 & 39.50 & 72.95 & 75.07 & 88.47 & 84.13 &  72.0 \\
          \textbf{all-MiniLM-L6-v2 (384)} & 81.44 & 42.99 & 75.98 & 80.56 & 91.80 & 87.38 &  90.0 \\
\bottomrule
\end{tabular}
\end{table*}
